Uncovering Cross-Domain Recommendation Ability of Large Language Models

Cross-Domain Recommendation (CDR) seeks to enhance item retrieval in low-resource domains by transferring knowledge from high-resource domains. While recent advancements in Large Language Models (LLMs) have demonstrated their potential in Recommender Systems (RS), their ability to effectively transfer domain knowledge for improved recommendations remains underexplored. To bridge this gap, we propose LLM4CDR, a novel CDR pipeline that constructs context-aware prompts by leveraging users' purchase history sequences from a source domain along with shared features between source and target domains. Through extensive experiments, we show that LLM4CDR achieves strong performance, particularly when using LLMs with large parameter sizes and when the source and target domains exhibit smaller domain gaps. For instance, incorporating CD and Vinyl purchase history for recommendations in Movies and TV yields a 64.28 percent MAP 1 improvement. We further investigate key factors including source domain data, domain gap, prompt design, and LLM size, which impact LLM4CDR's effectiveness in CDR tasks. Our results highlight that LLM4CDR excels when leveraging a single, closely related source domain and benefits significantly from larger LLMs. These insights pave the way for future research on LLM-driven cross-domain recommendations.

==> table/table-domain-diversity.tex <==
\begin{table}[t!]
\caption{Filtered cross-domain dataset statistics for domain diversity influence analysis.}
%\resizebox{1.0\textwidth}{!}{%
\scriptsize
\resizebox{0.98\columnwidth}{!}{
\fontsize{9}{10}\selectfont
\begin{tabular}{c|c|cc}
\toprule
Source & Target & \#User & Avg. Len. \\\hline
Video Games, CD \& Vinyl & Movies \& TV & 699 & 101.85 \\
Movies \& TV, Video Games & CD \& Vinyl & 623 & 323.81 \\
CD \& Vinyl, Movies \& TV & Video Games& 346 & 2053.05 \\
\bottomrule
\end{tabular}}%
% }
\label{table:domain-diversity}
\end{table}
